Building Very Small Test Suites (with Snap)

Software is now so large and complex that additional architecture is needed to guide theorem provers as they try to generate test suites. For example, the SNAP test suite generator (introduced in this paper) combines the Z3 theorem prover with the following tactic: sample around the average values seen in a few randomly selected valid tests. This tactic is remarkably effective. For 27 real-world programs with up to half a million variables, SNAP found test suites which were 10 to 750 smaller times than those found by the prior state-of-the-art. Also, SNAP ran orders of magnitude faster and (unlike prior work) generated 100% valid tests.

==> replies-v1.tex <==
\clearpage
\renewcommand{\thefigure}{R\arabic{figure}}
\setcounter{figure}{0}
\pagenumbering{roman}
\setcounter{page}{1}
\section*{Replies to Reviewers}
\subsection*{Associate Editor}

Reviewers pointed out several important problems in the (a) motivation, (b) approach design (e.g., use of the NCD measure) which should be carefully addressed in the revision.

\BLUE
Thank you for the opportunity to revise this document.  We have carefully studied
the reviewer comments. In the following,
we describe how this draft
has been revised  to address their comments.
For all our additions to the text, please
see the colored text.

As to your specific comments mentioned above, please see:

~\\
\begin{tabular}{|p{.6in}p{.3in}p{2.1in}|}\hline
what &where& notes\\\hline
a. Motivation & \tion{why} & For better notes on our why we take this approach, please see our new motivation section in \tion{why}.\\\hline
b. Approach &\tion{term};& 
For more notes on our approach, please see the new abstract and introduction test that takes greater care to explain the motivation and background to this work.

Also, please see   many places around the paper where we (e.g.)
including our new tutorial on NCD in \tion{term};\\\hline
c. Other &\tion{valid1}   \tion{valid2} &
Also, based on some insightful comments from the reviewers, we now have an extended and improved ``threats to validity'' section which serves to (much) better
scope our claims (see \tion{valid1} and \tion{valid2}).\\\hline
\end{tabular}

\BLACK
 
\subsection*{Reviewer1}



This paper presents a technique (named SNAP) attempting to improve a recently proposed technique named QuickSampler, which aims to generate a set of solutions satisfying a given set of SAT constraints in the CNF format. Like QuickSampler, SNAP uses the XOR operation on existing solutions to find new solutions to avoid time-consuming solving of the SAT constraints. Unlike QuickSampler, SNAP also uses a diversity measure named NCD to lead a search procedure for finding new solutions. SNAP is evaluated on the same set of SAT instances as QuickSampler.

In general, I think the proposed SNAP technique is interesting, since it seems much faster than QuickSampler. However, I have some serious concerns with the manuscript in the current form.


\BLUE
Thank you for your comments. We appreciate the detailed analysis of our work. Based on your feedback, we have added over a page of new text to this document, and made numerous changes around the paper.
To see all those changes,   please
see the colored text.
\BLACK




\subsubsection*{1a: Misleading?}
It is misleading that the manuscript implies in the beginning that general test generation for software testing can be represented as generating a set of inputs satisfying a given set of constraints. In fact, typical test generation in software testing requires generating test inputs satisfying different sets of constraints, where each set of constraints corresponds to an execution path. Of course, in some cases (e.g., where there are constraints that cannot be handled by the used solver), we may need to generate multiple inputs satisfying a set of constraints representing a common path prefix. I think this issue should be carefully handled in the manuscript; otherwise, readers may misunderstand the proposed technique.

\BLUE
  Thank you for your comment -- and we agree
that the previous version of the paper was
far too general in its claims.

We can see several cases where your comment implies limitations on {\sc Snap}. We have listed those cases in new subsections
within ``Threats to Validity'' (see \tion{valid1}
and \tion{valid2}) where we expand on your comments above.

% We hope  that, when you read~\tion{valid1}
% and \tion{valid2} that
% you  see we have taken care to document and extend your argument in the current text. 
% But also, we
%  hope that you think (as we do)
% that even though{\sc Snap} has the limitations
% documented in~\tion{valid1}
% and \tion{valid2}, the current functionality is still a significant extension to
% the prior state of the art work. 

 
\BLACK

\subsubsection*{1b: NCD}The use of the NCD measure in solution generation is questionable.  It is unclear what the NCD means for SAT solutions. 

\BLUE
You are correct -- the previous
draft did not explain NCD is sufficient detail.

\tion{term} now includes a more extensive tutorial on NCD.

Please accept our apologies for not including those details in
the last version.
\BLACK



\subsubsection*{1c: NCD (again)} Second, there may be some intrinsic shortcoming of the NCD measure. Given a set of solutions (denoted as X), if there exists a solution (denoted as s) in X such that C(s) is close to 0, the value of the NCD measure would probably become close to 1 (i.e., (C(X)-C(s))/C(X-{s}) precisely). No matter what other solutions in X are, the NCD may be the same.

\BLUE
You are completely correct "like any normalization function NCD could "explode" in the case of values close to 0.
But regarding to the NCD for test suites, we want to make two comments:
\bi
\item Even though there exists some test cases $s$ where $C(x)=0$, it does not imply that the NCD of whole test suite become close to 1. \tion{term} has more context on this.
\item We have checked our logs. We did not see such close-to-zero values. To show this, we calculated the distribution of $C(x)$ where $x$ is the test cases yield at the end of our experiment. \fig{cx_dist}  (on the next page) plots the distributions in four benchmarks.
\ei
\BLACK
\begin{figure*}[!tb]
\begin{center}    
\includegraphics[width=.245\textwidth]{cx_1.pdf}
\includegraphics[width=.245\textwidth]{cx_2.pdf}   
\includegraphics[width=.245\textwidth]{cx_3.pdf}   
\includegraphics[width=.245\textwidth]{cx_4.pdf} 
\end{center}
\caption{\BLUE Distributions of $C(x)$ for the test suite in various benchmarks, where $x$ is the test cases in the suite and $C(x)$ is one component of NCD calculation {\it(see \tion{term} for the definition)}. To demonstrate we did not see close-to-zero $C(x)$, we let x-axis always start from 0. See replies 1c for details.
\BLACK
}\label{fig:cx_dist}
\end{figure*}


\subsubsection*{1d: Uniformity vs Diversity} An important measure (i.e., uniformity of coverage) used for evaluating existing techniques for generating solutions for a set of SAT constraints is not adopted in evaluating SNAP. 

\BLUE
Thank you for that comment.
We note that 
we did try to repeat the uniformity
analysis of the QuickSampler paper  in \tion{abias}. But, as noted in that section,
there were some technical reasons why we could not exactly repeat that analysis.
What we could show, in \tion{abias}, 
was that if solutions were generated by {\em QuickSampler} with a particular entropy (which is an indicator for uniformity), then it is likely that the {\sc Snap} would generating  that  kind  of  solutions  
as  well.  

That said, we completely agree with your more general point that we needed to better describe why we selected the particular  the evaluation criteria used in this paper.  The first column of the
new introduction now offers much more detail on that point. Also, in \tion{eval} we describe several
evaluation methods we did not explore. 
There are numerous many ways that this
kind of reasoning could be evaluated (including uniformity). Since no
 paper can explore all evaluation
criteria, 
what we have done here is carefully explain all our definitions and made our tools open source. In this way, our methods could be tested by the community or a  wide variety of criteria.

Finally, please note that our  new  \tion{eval}
ends with an extensive
discussion on why, when
targeting very large test
suite reduction, it may be preferable to explore
issues other than uniformity.
 
% Another reason not pursue uniformity as a primary goal is that it does not match
%  the  goals of our industrial partners.
% In \tion{why}, we have added extensive notes on the business case
% presented to use by our industrial partners (see the end of   \tion{why}).
% We have tried explain uniformity and diversity to that industrial community
% and must report that it is not an issue that concerns them.
% Our industrial partners asked for a variant
% of that system that fund fewer tests.
% When we asked them about uniformity or diversity,
% there answer was always ``whatever gets us to fewer tests''. 



\BLACK
\subsubsection*{1e:  What is the goal of this work?}
In summary, if the authors aim for a technique for general software testing, the authors should provide evidence on some real software systems that  test suites generated by SNAP are preferable compared with some existing test generation technique; 

\BLUE
This is a good point. We agree that the goals of this work were not probably stated in the prior
draft. Rather than tackle the very general problem of building a test
suite generator ``for general software testing'' (to use your expression),
this draft takes much greater care to
restrict its target. Specifically:
\bi
\item
\tion{valid1} and \tion{valid2}
defines four kinds of testing
and notes the {\sc Snap} is best suited to  one of those.
\item In the first column of our introduction we defined five criteria 
(runtime, scalability, redundancy, credibility and minimality) and note that
{\em QuickSampler} needs to be improved on three of those criteria (redundancy, credibility and minimality). The rest of the paper then evaluates {\sc Snap} on those criteria.
\ei

\BLACK
\subsubsection*{1f:  Minor issues}

There are some typos in the manuscript. 

\BLUE
 Thanks for the fix.  To fix the typo you mention, and others, this version has been proofread by several people.
\BLACK



 
 \subsection*{Reviewer2}

In the paper, the authors deal with improving test suite generation based on a constraint representation of a program and constraint solving. When understanding the paper right, the constraint representation (more or less) captures the path conditions of the program, and test cases are supposed to fulfill these conditions. The content of the paper is based on previous work in this direction. The proposed improvement is based on a specific tactics that leads to a substantially reduced test set, which is a very good contribution worth being published.

  The paper itself, is well structured and also well explained.

\BLUE
Thank you for your comments -- we found them very pertinent and very useful.
To see the changes we made in response to your comments, 
please
see the sections in blue.

Also, we hope you don't mind, we reorganized your comments for the sake of brevity
into your two themes which were 
\bi
\item Be clearer: get to the point;
\item
Do not say ``more valid''.
 \ei
 
\BLACK
\subsubsection*{2a: Be clearer: get to the point}
After reading the paper it seems that the authors would be able to explain their approach using far less pages... 
 In order to improve the paper, the authors should consider using focusing more on the approach and its comparison and make the paper also shorter. ...
 The discussion about the time required for repairing vs.generating  vs.  verifying  is  fine  but  rather  obvious  because  this is more or less depending on the number of variables where we are searching for values. Verifying whether a specific setting of values to variables is satisfiable is not time consuming. Having only a subset of the variables to be searched for (like in the case of  repairing)  we  need  less  time.  Hence,  the  whole  discussion seems  to  be  trivial.

 
 

\BLUE
  Thank you for your comments. We agree that the last version could be shortened. Specifically,
  before adding in the material requested
  by other reviewers, we first pruned  1.5 pages from the last draft
  In this version:
\bi
\item
We have cut back most of the superfluous notes in the introduction .
\item
We   removed a discussions section (that no reviewer cared about) that included
the parts that you, quite correctly, describe as trivial.
\item
There are are also some notes on repeated structure and backdoors which
we found interesting but, as you say, do not really add to the paper.
\ei
Note that:
\bi
\item
We could not shorten the {\em Related Work} section since the TSE
EIC wanted notes there to distinguish this work from something we'd done previously (the DODGE system).
\item
Also, reviewer1 needed some additional material added (about a page-- see the new notes in {\em External Validity}). Hope that's ok.
\ei
\BLACK
\subsubsection*{2b: Do not say ``more valid''.}

     RQ3 leads to an answer stating that the obtained tests are more valid. The terminology more valid seems to be somehow strange. Either a logical sentence or a set of constraints is valid (or satisfiable) or not. Hence, it seems that some of the tests computed using QuickSampler are not valid (which is bad) but the new approach only provides valid tests (which is good).
  
  

\BLUE
  You are quite. ``More valid'' is just the wrong thing to say. Now
  we say ``more credible'' which in the introduction, we define as follows:
  \begin{quote} {\em 
   We say  that  one  test  suite  is  ``more  credible''  than  another  if  it contains  a  large  percentage  of  tests  that  are  valid  (satisfy  local domain  constraints).   }
\end{quote}
 
This draft now replaces ``more valid'' with ``more credible'':
see the Introduction and \tion{validity} and the new $x$-axis label
for \fig{hit}.
\BLACK
   
 
\subsection*{Reviewer: 3}

This paper proposes SNAP, a test suite generator that combines the Z3 theorem prover with a generation tactic that considers that code has much repeated structure. The authors motivate the generation of small test suites with the time spent by developers in (a) analysing what should be the required output; and (b) debugging failed tests.

 The way this paper is written make it an easy and joyful read.

\BLUE
Thank you. That is so humbling--  we have never had a such comment before.   

In reply, we thank you for the clarity
of your review. Your comments 
pointed us to a major flaw in the last draft.
Your insight was that the prior draft motivated
itself with A,B,C then evaluated itself using
X,Y,Z.  This has now been fixed.  
\BLACK

\subsubsection*{3a: Motivation}
My main comment with respect to this paper is about the motivation mentioned above. Again, the authors motivate the generation of small test suites with the time spent by developers in (a) analysing what should be the required output; and (b) debugging failed tests. However, the empirical evaluation does not answer (a) nor (b). I would have liked the authors to have two research questions to study the evidence that the motivation is indeed correct.

\BLUE
Thank you for that comment. You are completely correct- the Introduction of the prior draft    offered
the wrong motivation for the paper.
Accordingly,
in this new draft:
\bi
\item
The Introduction offers a motivation that actually corresponds to what we did in our experiments; i.e. we
wish to reduce the redundancy, credibility and minimality problems associated with {\em QuickSampler}.
\item
The old motivation (is now moved to \tion{why}). Here, we take care to start that section with a paragraph stressing that we will be assessing {\sc Snap}
using criteria from the introduction. 
\ei
\BLACK

\subsubsection*{3b: No Single Sentence Sections}

I personally do not like to see sections with just one subsection (as it is done in the Introduction). I would suggest to drop the subsection, but still include the text as a well defined paragraph.


\BLUE
Done!
\BLACK


\subsubsection*{ 3c: Compare with Perez?}
 Section 3.2: Perez et al. proposed recently at ICSE17 a test-suite diagnosability metric, which might be an interesting metric to consider as it maximizes test suites so that if something fails than there is enough information to diagnose the potential issue. The metric also explores structure's diversity. It would be off added value to re-do the experiments with this metrics too, or instead perhaps discuss it would be interesting and worth it. 

\BLUE
You raise an interesting point. There are very many different ways 
we might select to assess test case prioritization. A new \tion{eval} of this
paper discusses some of these methods, including the  Perez et al. method you mentioned above.

% Both SNAP  or {\it QuickSampler} in previous paper,
% did not discuss the efficiency of fault localization in the benchmarks. This is because those benchmarks were
% extracted and transformed from real-world hardware or giant software systems. We did not have the resource to find out the obtained errors given the test suite. Therefore, we can only focus on
% the diversity, uniformity or other metrics in the test suite itself, instead of the obtained errors after executing them.


As to the particular comparisons you suggest,
  (with the Perez metrics), that  would not just comment
on {\sc Snap} but also {\em QuickSampler} all prior work that used theorem provers to generate test suites. We do not doubt that that would be an insightful analysis -- it could  indeed be interesting and insightful to  repeat this study using the Perez metrics in other smaller benchmarks (so that we can obtain executing results of the test suites).
But
our feeling is that that would be worthy of an entirely separate paper.


Also, we do have some systems issues with doing the comparison you propose. The former grad student who worked on this (Dr. Chen, the first author) is now a full time research scientist at Facebook. And the grant that funded
Dr. Chen has terminated. Hence, at this time, we do not have the resources
to address this point.

So please advise: is your recommendation here a requirement for publication?  
We will of course work at your direction but it many take some months
to get the funds (and train the graduate student) needed to complete this task.
\BLACK



\subsubsection*{3d: Hyper parameters}

Section 3.3 is rather weak. All those control parameters are not well motivated and its impact should be discussed and empirically validated.

 \BLUE
You are quite correct -- we did not discuss hyper parameter optimization
in this domain, Please see the notes in \tion{hpo}. In summary,
due to the long run-times of our systems, it would be an exciting and challenging
problem to improve our current results.

That said, what is true is  that our current system clearly out-performs a
recent state-of-the-art publication from ICSE'18.  So while hyperparameter optimization would clearly be interesting, we feel we have proved our
point that the {\sc Snap} tactic is useful.

But what is your view?

\BLACK


\subsubsection*{3f: Issues with the reproduction package}

. There are a few typos in the  README.md of the replication package:
    * replies --> relies 
    * avaialbel --> available 

Also, bout the replication package: (1) It was not straightforward for me to install and use the tool. Providing a container (docker, for instance) would help a great deal. (2) are the benchmarks included?


 \BLUE
 Thank you for your comments. Those typos
 have been fixed. Also:
 
1) An easy install {\it Makefile} is  now
included in the github repo. Also,
step by step installation can now can be found at \url{https://github.com/ai-se/SatSpaceExpo}.

2) The benchmarks are not included in the {\it SatSpaceExpo} repo; however, one can download it via \url{https://github.com/RafaelTupynamba/quicksampler/tree/master/Benchmarks}. Users should not worry about this if they're following step-by-step guidance now.
\BLACK
 

\subsubsection*{3g: nitpicking}

 in reference [3]: sat --> SAT.
 
 \BLUE
This was probably due the automatic formatting in {\tt \textbackslash bibliographystyle\{IEEEtran\}}. We've fixed all similar occurrences.
 \BLACK


